Angular analysis of the low $K^{+}K^{-}$ invariant mass enhancement in $B^{+}\to K^{+}K^{-}\pi^{+}$ decays

We study the decay $B^{+} \to K^+ K^- \pi^+$ and investigate the angular distribution of $K^{+}K^{-}$ pairs with invariant mass below $1.1$ GeV/$c^2$. This region exhibits both a strong enhancement in signal and very large direct $CP$ violation. We construct a coherent sum model for the angular distribution of $S$- and $P$-wave, and report the ratio of their amplitudes, the relative phase and the forward-backward asymmetry. We also report absolute differential branching fractions and direct $CP$ asymmetry for the decay in bins of $M_{K^+K^-}$ and the differential branching fractions in bins of $M_{K^+\pi^-}$. The results are based on a data sample that contains $772\times10^6$ $B \bar{B}$ pairs collected at the $\Upsilon(4S)$ resonance with the Belle detector at the KEKB asymmetric-energy $e^+ e^-$ collider. The measured overall branching fraction and the direct $CP$ asymmetry are $(5.38\pm0.40\pm0.35)\times 10^{-6}$ and $-0.170\pm0.073\pm0.017$, respectively, where the first uncertainties are statistical and the second are systematic.

==> pub592-orcid.tex <==
%%% Paper:    B+ to K+ K- pi+
%%% Journal:  Physical Review D
%%% Contacts: C.-L. Hsu (chia-ling.hsu@sydney.edu.au)
%%%           D. Dossett (david.dossett@unimelb.edu.au)
%%% Non-responding authors or those who said NO are commented out.
%%% ====================================================================
%%% Click the RELOAD button on your web browser to see the updated file.
%%% ====================================================================
%%% Use \input{author-orcid} to insert this material into your latex file.
%%%%% Force institutions to appear in alphabetical order when typeset.
\noaffiliation
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
% \author{A.~Abdesselam\,\orcidlink{-}} % -583
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{S.~Al~Said\,\orcidlink{0000-0002-4895-3869}} % 6823
% \author{K.~Arinstein\,\orcidlink{-}} % -87
% \author{Y.~Arita\,\orcidlink{-}} % -272
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
  \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
  \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290}} % 3766
% \author{T.~Aziz\,\orcidlink{-}} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
  \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
% \author{Y.~Ban\,\orcidlink{-}} % 3503
% \author{E.~Barberio\,\orcidlink{-}} % -229
% \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
  \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{P.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
% \author{C.~Bele\~{n}o\,\orcidlink{-}} % -582
  \author{K.~Belous\,\orcidlink{0000-0003-0014-2589}} % 2329
  \author{J.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
% \author{F.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
% \author{D.~Besson\,\orcidlink{-}} % 3585
  \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
  \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{J.~Biswal\,\orcidlink{0000-0001-8361-2309}} % -218
  \author{T.~Bloomfield\,\orcidlink{0000-0001-9288-5069}} % 2418
  \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
% \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
% \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
% \author{F.~Breibeck\,\orcidlink{-}} % 2247
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
% \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
% \author{G.~Caria\,\orcidlink{-}} % 2438
  \author{D.~\v{C}ervenkov\,\orcidlink{0000-0002-1865-741X}} % 2078
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
% \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
% \author{Y.~Chao\,\orcidlink{0000-0002-5976-318X}} % 14683
  \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
  \author{A.~Chen\,\orcidlink{0000-0002-8544-9274}} % -284
% \author{K.-F.~Chen\,\orcidlink{-}} % -298
% \author{Y.~Chen\,\orcidlink{0000-0002-2057-1076}} % 2576
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{H.~E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
% \author{V.~Chobanova\,\orcidlink{-}} % -560
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{Y.~Choi\,\orcidlink{0000-0003-3499-7948}} % -405
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
  \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
  \author{S.~Cunliffe\,\orcidlink{0000-0003-0167-8641}} % 2272
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
  \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
  \author{N.~Dash\,\orcidlink{0000-0003-2172-3534}} % 2601
  \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
  \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
  \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
% \author{Z.~Dr\'asal\,\orcidlink{-}} % -551
  \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
% \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
  \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
% \author{M.~Feindt\,\orcidlink{-}} % -532
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
  \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
% \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
  \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
  \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
% \author{M.~Gelb\,\orcidlink{-}} % 2340
% \author{J.~Gemmler\,\orcidlink{-}} % 2321
% \author{D.~Getzkow\,\orcidlink{-}} % 2416
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
% \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
% \author{J.~Grygier\,\orcidlink{-}} % 2313
  \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
% \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
% \author{E.~Guido\,\orcidlink{-}} % 2225
% \author{H.~Guo\,\orcidlink{-}} % -385
% \author{J.~Haba\,\orcidlink{-}} % 2222
  \author{C.~Hadjivasiliou\,\orcidlink{0000-0002-2234-0001}} % 9503
  \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
% \author{P.~Hamer\,\orcidlink{-}} % -580
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
  \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
  \author{O.~Hartbrich\,\orcidlink{0000-0001-7741-4381}} % 2158
% \author{J.~Hasenbusch\,\orcidlink{-}} % -234
  \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
% \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
% \author{X.~H.~He\,\orcidlink{-}} % -362
% \author{M.~Heck\,\orcidlink{-}} % 2561
% \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
% \author{D.~Heffernan\,\orcidlink{-}} % -334
% \author{M.~Heider\,\orcidlink{-}} % -534
% \author{A.~Heller\,\orcidlink{-}} % -541
% \author{M.~Hernandez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
% \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
% \author{K.~Hoshina\,\orcidlink{-}} % -493
  \author{W.-S.~Hou\,\orcidlink{0000-0002-4260-5118}} % -288
% \author{Y.~B.~Hsiung\,\orcidlink{-}} % -289
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
% \author{M.~Huschle\,\orcidlink{-}} % -535
% \author{Y.~Igarashi\,\orcidlink{-}} % 3644
% \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
% \author{M.~Imamura\,\orcidlink{-}} % -273
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
% \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{-}} % 4323
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
  \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
% \author{H.~B.~Jeon\,\orcidlink{0000-0002-0857-0353}} % 2170
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
% \author{D.~Joffe\,\orcidlink{-}} % 2295
  \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
% \author{T.~Julius\,\orcidlink{-}} % -232
% \author{J.~Kahn\,\orcidlink{0000-0002-8517-2359}} % 2448
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
  \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
% \author{J.~H.~Kang\,\orcidlink{-}} % -517
  \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
% \author{P.~Kapusta\,\orcidlink{0000-0003-1235-1935}} % 6663
% \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{S.~U.~Kataoka\,\orcidlink{-}} % 13483
% \author{Y.~Kato\,\orcidlink{0000-0001-6314-4288}} % 2549
% \author{H.~Kawai\,\orcidlink{-}} % 4344
% \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
% \author{T.~Keck\,\orcidlink{-}} % 2300
% \author{H.~Kichimi\,\orcidlink{0000-0003-0534-4710}} % 2233
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
  \author{C.~H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
% \author{H.~J.~Kim\,\orcidlink{0000-0001-9787-4684}} % 4863
% \author{H.-J.~Kim\,\orcidlink{-}} % 2691
% \author{J.~B.~Kim\,\orcidlink{-}} % 2408
% \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{K.~T.~Kim\,\orcidlink{0000-0003-2884-6772}} % 2409
% \author{S.~H.~Kim\,\orcidlink{-}} % 2428
% \author{S.~K.~Kim\,\orcidlink{-}} % 3823
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
  \author{T.~D.~Kimmel\,\orcidlink{0000-0002-9743-8249}} % 2241
% \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
% \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
% \author{C.~Kleinwort\,\orcidlink{0000-0002-9017-9504}} % 2499
% \author{J.~Klucar\,\orcidlink{-}} % -216
% \author{N.~Kobayashi\,\orcidlink{-}} % -546
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
% \author{Y.~Koga\,\orcidlink{-}} % -245
% \author{I.~Komarov\,\orcidlink{0000-0001-6282-1881}} % 2210
  \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
% \author{J.-F.~Krohn\,\orcidlink{0000-0002-5001-0675}} % 2502
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
% \author{B.~Kronenbitter\,\orcidlink{-}} % -540
  \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
  \author{R.~Kulasiri\,\orcidlink{0000-0002-0670-3968}} % 2441
% \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
% \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
% \author{E.~Kurihara\,\orcidlink{-}} % -95
% \author{Y.~Kuroki\,\orcidlink{-}} % -343
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
  \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
% \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
% \author{I.~S.~Lee\,\orcidlink{0000-0002-7786-323X}} % 2422
% \author{J.~K.~Lee\,\orcidlink{0000-0001-6397-0723}} % 2190
% \author{J.~Y.~Lee\,\orcidlink{0000-0003-3065-6118}} % 2596
  \author{S.~C.~Lee\,\orcidlink{0000-0002-9835-1006}} % 2544
% \author{R.~Leitner\,\orcidlink{-}} % -552
% \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
% \author{P.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
% \author{C.~H.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
% \author{H.~Li\,\orcidlink{-}} % -119
  \author{J.~Li\,\orcidlink{0000-0001-5520-5394}} % 11064
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{L.~Li~Gioi\,\orcidlink{0000-0003-2024-5649}} % 2495
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
  \author{K.~Lieret\,\orcidlink{0000-0003-2792-7511}} % 2268
% \author{A.~Limosani\,\orcidlink{-}} % -221
% \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
% \author{C.~Liu\,\orcidlink{-}} % -384
% \author{Y.~Liu\,\orcidlink{-}} % 10543
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
% \author{R.~Louvot\,\orcidlink{-}} % -205
% \author{M.~Lubej\,\orcidlink{-}} % 2513
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
% \author{J.~MacNaughton\,\orcidlink{-}} % -550
  \author{C.~MacQueen\,\orcidlink{0000-0002-6554-7731}} % 2585
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
  \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
  \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
  \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
% \author{Y.~Miyachi\,\orcidlink{-}} % -548
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
% \author{H.~Miyata\,\orcidlink{0000-0002-1026-2894}} % 2071
% \author{Y.~Miyazaki\,\orcidlink{-}} % -257
  \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
% \author{H.~K.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
% \author{T.~J.~Moon\,\orcidlink{0000-0001-9886-8534}} % 2397
% \author{T.~Mori\,\orcidlink{-}} % -264
% \author{T.~Morii\,\orcidlink{-}} % 3543
% \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
% \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{T.~M\"uller\,\orcidlink{0000-0003-4337-0098}} % 2165
% \author{N.~Muramatsu\,\orcidlink{-}} % -549
% \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
% \author{Y.~Nagasaka\,\orcidlink{-}} % -138
% \author{Y.~Nakahama\,\orcidlink{-}} % -466
% \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328}} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
% \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
% \author{T.~Nanut\,\orcidlink{-}} % 2565
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
  \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
  \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
% \author{C.~Ng\,\orcidlink{-}} % -467
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
  \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
  \author{N.~K.~Nisar\,\orcidlink{0000-0001-9562-1253}} % 2522
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
% \author{O.~Nitoh\,\orcidlink{-}} % -491
% \author{A.~Ogawa\,\orcidlink{-}} % -116
% \author{K.~Ogawa\,\orcidlink{0000-0003-2220-7224}} % 2430
  \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
% \author{T.~Ohshima\,\orcidlink{-}} % -237
% \author{S.~Okuno\,\orcidlink{-}} % -164
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
  \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
  \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{W.~Ostrowicz\,\orcidlink{0000-0003-1434-4608}} % 3983
% \author{C.~Oswald\,\orcidlink{-}} % -233
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
  \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
% \author{B.~Pal\,\orcidlink{0000-0003-0737-1528}} % 2274
% \author{T.~Pang\,\orcidlink{0000-0003-1204-0846}} % 2114
% \author{E.~Panzenb\"ock\,\orcidlink{-}} % -581
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
% \author{C.-S.~Park\,\orcidlink{-}} % 2307
% \author{C.~W.~Park\,\orcidlink{-}} % -411
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
% \author{K.~S.~Park\,\orcidlink{-}} % -409
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
% \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
% \author{T.~Peng\,\orcidlink{-}} % -387
% \author{L.~Pes\'{a}ntez\,\orcidlink{-}} % -235
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
% \author{M.~Peters\,\orcidlink{-}} % -122
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
% \author{K.~Prasanth\,\orcidlink{-}} % 2383
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
% \author{K.~Prothmann\,\orcidlink{-}} % -555
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
% \author{A.~Rabusov\,\orcidlink{0000-0001-8189-7398}} % 2355
% \author{J.~Rauch\,\orcidlink{-}} % 2536
% \author{B.~Reisert\,\orcidlink{-}} % -556
% \author{E.~Ribe\v{z}l\,\orcidlink{-}} % -217
% \author{M.~Ritter\,\orcidlink{0000-0001-6507-4631}} % 2580
% \author{M.~R\"{o}hrken\,\orcidlink{0000-0003-0654-2866}} % 11883
  \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
  \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
  \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
% \author{M.~Salehi\,\orcidlink{-}} % 2127
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
  \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
% \author{D.~Santel\,\orcidlink{-}} % -105
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
  \author{T.~Sanuki\,\orcidlink{0000-0002-4537-5899}} % 6783
% \author{J.~Sasaki\,\orcidlink{-}} % 4383
% \author{N.~Sasao\,\orcidlink{-}} % -192
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
% \author{T.~Schl\"{u}ter\,\orcidlink{-}} % -545
% \author{O.~Schneider\,\orcidlink{-}} % -198
  \author{G.~Schnell\,\orcidlink{0000-0002-7336-3246}} % 12204
% \author{M.~Schram\,\orcidlink{-}} % 2306
  \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
% \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{R.~Seidl\,\orcidlink{0000-0002-6552-6973}} % -115
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
% \author{D.~Semmler\,\orcidlink{-}} % -111
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
% \author{O.~Seon\,\orcidlink{-}} % 2581
% \author{L.~Shang\,\orcidlink{-}} % -142
  \author{M.~Shapkin\,\orcidlink{0000-0002-4098-9592}} % 2460
  \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
  \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
% \author{T.-A.~Shibata\,\orcidlink{-}} % -547
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
% \author{S.~Shinomiya\,\orcidlink{-}} % -342
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
  \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
% \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
% \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
% \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
% \author{R.~Sinha\,\orcidlink{-}} % 3423
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381}} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
% \author{M.~Steder\,\orcidlink{-}} % 2153
  \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
% \author{J.~F.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
% \author{J.~Stypula\,\orcidlink{0000-0002-5844-7476}} % 2368
% \author{S.~Sugihara\,\orcidlink{-}} % -468
% \author{A.~Sugiyama\,\orcidlink{-}} % -376
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
  \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
  \author{T.~Sumiyoshi\,\orcidlink{0000-0002-0486-3896}} % 4184
% \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
% \author{K.~Suzuki\,\orcidlink{-}} % 2445
% \author{S.~Suzuki\,\orcidlink{-}} % -377
% \author{S.~Y.~Suzuki\,\orcidlink{0000-0002-7135-4901}} % 2496
% \author{H.~Takeichi\,\orcidlink{-}} % -246
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
  \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{M.~Tanaka\,\orcidlink{-}} % 4246
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
  \author{Y.~Tao\,\orcidlink{0000-0002-9186-2591}} % 2362
% \author{G.~N.~Taylor\,\orcidlink{-}} % -220
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
% \author{Y.~Teramoto\,\orcidlink{0000-0002-1738-6697}} % -349
% \author{A.~Thampi\,\orcidlink{-}} % 7403
% \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
% \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
% \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
% \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
% \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
% \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
% \author{Y.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
% \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
% \author{C.~Van~Hulse\,\orcidlink{-}} % -579
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816}} % 2706
% \author{P.~Vanhoefer\,\orcidlink{-}} % -559
  \author{G.~Varner\,\orcidlink{0000-0002-0302-8151}} % 2119
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
% \author{K.~Vervink\,\orcidlink{-}} % -206
  \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
% \author{V.~Vorobyev\,\orcidlink{0000-0002-6660-868X}} % 2298
% \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
% \author{M.~N.~Wagner\,\orcidlink{-}} % -110
  \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
  \author{C.~H.~Wang\,\orcidlink{0000-0001-6760-9839}} % 2224
% \author{D.~Wang\,\orcidlink{0000-0003-1485-2143}} % 10003
  \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
% \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
% \author{P.~Wang\,\orcidlink{-}} % -150
  \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
  \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
% \author{Y.~Watanabe\,\orcidlink{-}} % -165
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{R.~Wedd\,\orcidlink{-}} % -231
% \author{S.~Wehle\,\orcidlink{0000-0002-6168-1829}} % 2489
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
% \author{E.~Widmann\,\orcidlink{-}} % -509
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
  \author{X.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
% \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
% \author{H.~Yamamoto\,\orcidlink{-}} % 2964
% \author{Y.~Yamashita\,\orcidlink{-}} % -323
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
% \author{S.~Yashchenko\,\orcidlink{-}} % 2135
  \author{H.~Ye\,\orcidlink{0000-0003-0552-5490}} % 2537
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
% \author{Y.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
% \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
% \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
% \author{C.~C.~Zhang\,\orcidlink{-}} % -141
% \author{J.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
% \author{L.~M.~Zhang\,\orcidlink{-}} % -383
  \author{Z.~P.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
% \author{L.~Zhao\,\orcidlink{-}} % -386
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
  \author{V.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
% \author{T.~Zivko\,\orcidlink{-}} % -215
% \author{A.~Zupanc\,\orcidlink{-}} % 2543
% \author{N.~Zwahlen\,\orcidlink{-}} % -207
\collaboration{The Belle Collaboration}

